Adaptive Meta-learning-based Adversarial Training for Robust Automatic Modulation Classification

DL-based automatic modulation classification (AMC) models are highly susceptible to adversarial attacks, where even minimal input perturbations can cause severe misclassifications. While adversarially training an AMC model based on an adversarial attack significantly increases its robustness against that attack, the AMC model will still be defenseless against other adversarial attacks. The theoretically infinite possibilities for adversarial perturbations mean that an AMC model will inevitably encounter new unseen adversarial attacks if it is ever to be deployed to a real-world communication system. Moreover, the computational limitations and challenges of obtaining new data in real-time will not allow a full training process for the AMC model to adapt to the new attack when it is online. To this end, we propose a meta-learning-based adversarial training framework for AMC models that substantially enhances robustness against unseen adversarial attacks and enables fast adaptation to these attacks using just a few new training samples, if any are available. Our results demonstrate that this training framework provides superior robustness and accuracy with much less online training time than conventional adversarial training of AMC models, making it highly efficient for real-world deployment.

==> 2_related_work.tex <==
\section{Related Work}

Theoretically, maximum likelihood provides the Bayes-optimal solution for modulation classification, but it assumes {prior} knowledge of channel conditions, which are highly dynamic in real-world communication systems. DL models were proposed as an alternative solution for AMC \cite{o2017introduction} which can implicitly learn channel variations and adapt to them given sufficient amount of data. Since then, various DL architectures such as CNNs\cite{west2017deep}, DNNs, and LSTMs \fa{define acronyms} have been proposed and evaluated for AMC, demonstrating the superior performance of DL-based AMC models over traditional methods. 

Despite the strong performance of DL-based AMC methods, many researchers have pointed out their vulnerability to adversarial attacks \cite{sadeghi2018adversarial, lin2020threats, flowers2019evaluating}. These works have demonstrated that adversarial perturbations require significantly less power compared to AWGN to void AMC predictions. A couple of methods have been proposed as defensive mechanism for AMC models against adversarial perturbations such as randomized smoothing and data augmentation \cite{kim2021channel}, ensemble learning \cite{sahay2021deep}, and miss-classification correction \cite{sahay2021deep}. But arguably, adversarial training has been the most favored solution \cite{maroto2022safeamc,sahay2021robust}.

\fa{there is a large disconnect between these two paragraphs. we either need to discuss the cons of adversarial training-based AMC models and their cons which is the repeat of introduction OR we remove the related work, add its first paragraph to the intro and discuss [14] within the intro (others can be removed or moved to the proposed model, whre you add 2-3 sentence about prior meta-learning based PHY-layer works   }

One of the key factors that has largely remained neglected in DL-based works in wireless communication applications in general, is the ever-evolving and dynamic nature wireless channels which calls for retraining and fine-tuning the DL-based wireless models. Collecting data and training costs are usually constraining in a practical scenario, which calls for utilization of DL models with fast adaption capabilities. To this end, meta-learning has been proposed in more recent years as an alternative to the conventionally trained DL models in various wireless application such as, interference identification \cite{owfi2023meta}, channel autoencoders \cite{park2020meta}, and AMC \cite{hao2024meta, hao2023automatic} as well. In one of the recent works \cite{zhang2022spectrum} it is claimed that meta-learning is used to improve robustness of AMC to black-box attacks. But based on the pseudo-code and the objective functions provided in the paper, their proposed method is multi-task learning rather than meta-learning as the loss function simply uses the average loss of the model on multiple tasks. To the best of our knowledge, no paper has addressed the need for adaptive robust AMC models against new adversarial attacks using meta learning.


==> old_intro.tex <==
\section{Introduction}
% \fa{should we have online or a similar term in the title? }
% Since the integration of deep learning (DL) models into wireless communication systems, these models have demonstrated remarkable potential across a range of applications, including channel estimation, signal detection, and beamforming optimization. DL has proven particularly advantageous over traditional methods due to its ability to automatically extract complex features from raw data, adapt to dynamic environments in the presence of sufficient training data, and improve performance without relying on handcrafted features.

One of the most researched applications of DL-based solutions in wireless communications is automatic modulation classification (AMC). AMC involves identifying the modulation scheme of received signals, a crucial task for spectrum management, interference recognition and mitigation, and cognitive radio systems. The ability to automatically classify modulation schemes enables intelligent communication systems that can dynamically adapt to changing signal environments given sufficient training samples.


Despite the impressive performance of DL-based AMC models, and the considerable research papers focusing on this field, their widespread adoption in practical systems remains limited. A key challenge lies in the vulnerability of DL models to adversarial attacks, a concern that extends beyond wireless communications and affects DL applications in general. Adversarial attacks involve subtle perturbations to input data that can cause significant degradation in model performance.

In the context of AMC, sources of interference using adversarial perturbations can severely undermine the accuracy of AMC models. Although adversarial training—where the model is trained with adversarially perturbed examples—can significantly enhance robustness to observed attack types\cite{sahay2021robust,maroto2022safeamc}, these models will still remain vulnerable to unseen attack variations, e.g., attack perturbation not used in the adversarial training process. As theoretically there can be infinite attack variations, an AMC model should expect to encounter unseen types of attacks when deployed to a real-time online system. This highlights the need for resilient DL-based AMC models that rely on fast adaptation to unseen adversarial attacks rather than DL models relying on adversarial training using a handful of pre-defined attack variations.

Moreover, a common yet unrealistic assumption within the AMC literature is that the distribution of signals' data remains stationary \cite{flowers2019evaluating,maroto2022safeamc,kim2021channel}. These proposed AMC methods split a single dataset into a training set and testing and evaluate the model on the testing set that was sampled from the same distribution as the training set. This approach implicitly assumes that the wireless environment remains stationary over time, which often does not hold true in real-world applications. This is while the radio spectrum is highly dynamic and rapidly evolving in reality, demanding continuous adaptation and fine-tuning of the AMC model. Furthermore, most works also assume access to large amounts of annotated training samples, as well as ample training time and resources for an AMC model to train and adjust itself to wireless variations. In practice, however, AMC models are typically constrained by the limited availability of training samples and computational resources in real-time online scenarios. Limitations in the availability of training samples and training resources often results in a few-shot learning scenario, a factor largely neglected in the current AMC literature \cite{flowers2019evaluating,maroto2022safeamc,kim2021channel,o2017introduction,west2017deep}. 

We believe a more realistic depiction of how AMC models can be practically implemented aligns with the system model shown in Fig \ref{fig:AMC-offline-online}. In the offline phase, sufficient datasets, powerful computational resources resources, and ample training time are available for pre-training and preparing the AMc model. Most previous AMC papers only consider this offline phase. However, we additionally consider an online phase where the pre-trained model is deployed within a practical system. During the online phase, the AMC model has to adapt and fine-tune itself in response to dynamic variations in real-time. Unlike the offline phase, the AMC model is challenged with limited new training samples, training resources, and training time in the online phase.


\begin{figure}{}
        \centering
        \includegraphics[width=0.6\columnwidth]{figs/offline-online.png} % Replace with your image
        \caption{Limitations of AMC models after being deployed to a practical real-world system (online-phase).}
        \label{fig:AMC-offline-online}
        \vspace{-15pt}
 \end{figure}


% To enable AMC to be viable for real-world implementation, we propose a new adaptive adversarial training framework for AMC that allows robustness to unseen adversarial attacks. In our proposed framework, under the meta-learning paradigm, we adversarially train the AMC model with a collection of known adversarial attacks during the offline training phase. By utilizing meta-learning, our proposed AMC can adapt to become robust against unseen adversarial attacks using only a handful of training samples. To the best of our knowledge, we are the first to propose an adaptive adversarial training framework for AMC. In summary, the main contributions of this paper are as follows:

To address these limitations in prior work, we propose a meta-learning-based adversarial training framework for AMC models aimed at robustness against new adversarial attacks in the online phase. Unlike conventional adversarial training for AMC models, which focuses on resilience to specific pre-defined attack types, our approach equips the AMC model to learn a generalized adaptation strategy, which enables the model to rapidly adapt to new adversarial attacks using only a handful of adversarial samples. Even when there are no new training samples in the online phase, an AMC model can reach much better generalization in robustness against new adversarial attacks when our proposed meta-learning-based training framework is employed. Moreover, the low computational and minimal training sample requirements of our proposed framework in the online phase satisfy the constraints of deploying an AMC model in real time within a practical system. \textit{To the best of our knowledge, we are the first to propose an adversarial training framework for AMC capable of fast adaptation in the online phase.} In summary, the main contributions of this paper are as follows:



\ali{Please give me your feedback on the contributions}
\begin{itemize}
    
    \item Addressing the common unrealistic assumption of single training/testing phase in AMC models by proposing a two-phased offline-training/online-deployment scenario for AMC models.
    \item Proposing a practical adversarial training framework for AMC models, with increased generalized robustness, and capable of fast adaptation to new adversarial attacks in the online phase.
    \item Substantially increasing efficiency by lowering data and training requirements during online deployment.
      
\end{itemize}






% The rest of this paper is structured as follows: Section
% II discusses previous papers focusing on adversarial attacks in DL-based AMC models. Section III \blue{explain methodology}. In Section IV, experiment settings are explained and evaluations are provided.
% Finally, Section V concludes the paper.
